Improving self-supervised pretraining models for epileptic seizure detection from EEG data

There is abundant medical data on the internet, most of which are unlabeled. Traditional supervised learning algorithms are often limited by the amount of labeled data, especially in the medical domain, where labeling is costly in terms of human processing and specialized experts needed to label them. They are also prone to human error and biased as a select few expert annotators label them. These issues are mitigated by Self-supervision, where we generate pseudo-labels from unlabelled data by seeing the data itself. This paper presents various self-supervision strategies to enhance the performance of a time-series based Diffusion convolution recurrent neural network (DCRNN) model. The learned weights in the self-supervision pretraining phase can be transferred to the supervised training phase to boost the model's prediction capability. Our techniques are tested on an extension of a Diffusion Convolutional Recurrent Neural network (DCRNN) model, an RNN with graph diffusion convolutions, which models the spatiotemporal dependencies present in EEG signals. When the learned weights from the pretraining stage are transferred to a DCRNN model to determine whether an EEG time window has a characteristic seizure signal associated with it, our method yields an AUROC score $1.56\%$ than the current state-of-the-art models on the TUH EEG seizure corpus.

==> refs <==
@article{manna,
  title={Neural correlates of focused attention and cognitive monitoring in meditation},
  author={Manna, Antonietta and Raffone, Antonino and Perrucci, Mauro Gianni and Nardo, Davide and Ferretti, Antonio and Tartaro, Armando and Londei, Alessandro and Del Gratta, Cosimo and Belardinelli, Marta Olivetti and Romani, Gian Luca},
  journal={Brain research bulletin},
  volume={82},
  number={1-2},
  pages={46--56},
  year={2010},
  publisher={Elsevier}
}

@article{avitan2009eeg,
	title={EEG generator—a model of potentials in a volume conductor},
	author={Avitan, Lilach and Teicher, Mina and Abeles, Moshe},
	journal={Journal of neurophysiology},
	volume={102},
	number={5},
	pages={3046--3059},
	year={2009},
	publisher={American Physiological Society Bethesda, MD}
}

@inproceedings{wagh2020eeg,
  title={Eeg-gcnn: Augmenting electroencephalogram-based neurological disease diagnosis using a domain-guided graph convolutional neural network},
  author={Wagh, Neeraj and Varatharajah, Yogatheesan},
  booktitle={Machine Learning for Health},
  pages={367--378},
  year={2020},
  organization={PMLR}
}
@article{tzallas2009epileptic,
  title={Epileptic seizure detection in EEGs using time--frequency analysis},
  author={Tzallas, Alexandros T and Tsipouras, Markos G and Fotiadis, Dimitrios I},
  journal={IEEE transactions on information technology in biomedicine},
  volume={13},
  number={5},
  pages={703--710},
  year={2009},
  publisher={ieee}
}
@article{o2020neonatal,
  title={Neonatal seizure detection from raw multi-channel EEG using a fully convolutional architecture},
  author={O’Shea, Alison and Lightbody, Gordon and Boylan, Geraldine and Temko, Andriy},
  journal={Neural Networks},
  volume={123},
  pages={12--25},
  year={2020},
  publisher={Elsevier}
}
@article{shuman2013emerging,
  title={The emerging field of signal processing on graphs: Extending high-dimensional data analysis to networks and other irregular domains},
  author={Shuman, David I and Narang, Sunil K and Frossard, Pascal and Ortega, Antonio and Vandergheynst, Pierre},
  journal={IEEE signal processing magazine},
  volume={30},
  number={3},
  pages={83--98},
  year={2013},
  publisher={IEEE}
}
@article{acharya2016american,
  title={American clinical neurophysiology society guideline 2: guidelines for standard electrode position nomenclature},
  author={Acharya, Jayant N and Hani, Abeer J and Cheek, Janna and Thirumala, Parthasarathy and Tsuchida, Tammy N},
  journal={The Neurodiagnostic Journal},
  volume={56},
  number={4},
  pages={245--252},
  year={2016},
  publisher={Taylor \& Francis}
}
@article{jayarathne2020person,
  title={Person identification from EEG using various machine learning techniques with inter-hemispheric amplitude ratio},
  author={Jayarathne, Isuru and Cohen, Michael and Amarakeerthi, Senaka},
  journal={PloS one},
  volume={15},
  number={9},
  pages={e0238872},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA}
}
@article{raghu2020eeg,
  title={EEG based multi-class seizure type classification using convolutional neural network and transfer learning},
  author={Raghu, Shivarudhrappa and Sriraam, Natarajan and Temel, Yasin and Rao, Shyam Vasudeva and Kubben, Pieter L},
  journal={Neural Networks},
  volume={124},
  pages={202--212},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{wang2020sequential,
  title={A Sequential Graph Convolutional Network with Frequency-domain Complex Network of EEG Signals for Epilepsy Detection},
  author={Wang, Jialin and Liang, Shen and He, Dake and Wang, Ye and Wu, Yingpei and Zhang, Yanchun},
  booktitle={2020 IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
  pages={785--792},
  year={2020},
  organization={IEEE}
}
@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}
@article{bullmore2009complex,
  title={Complex brain networks: graph theoretical analysis of structural and functional systems},
  author={Bullmore, Ed and Sporns, Olaf},
  journal={Nature reviews neuroscience},
  volume={10},
  number={3},
  pages={186--198},
  year={2009},
  publisher={Nature Publishing Group}
}
@inproceedings{ahmedt2020neural,
  title={Neural memory networks for seizure type classification},
  author={Ahmedt-Aristizabal, David and Fernando, Tharindu and Denman, Simon and Petersson, Lars and Aburn, Matthew J and Fookes, Clinton},
  booktitle={2020 42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  pages={569--575},
  year={2020},
  organization={IEEE}
}
@article{banville2021uncovering,
  title={Uncovering the structure of clinical EEG signals with self-supervised learning},
  author={Banville, Hubert and Chehab, Omar and Hyv{\"a}rinen, Aapo and Engemann, Denis-Alexander and Gramfort, Alexandre},
  journal={Journal of Neural Engineering},
  volume={18},
  number={4},
  pages={046020},
  year={2021},
  publisher={IOP Publishing}
}
@inproceedings{tang2021self,
  title={Self-Supervised Graph Neural Networks for Improved Electroencephalographic Seizure Analysis},
  author={Tang, Siyi and Dunnmon, Jared and Saab, Khaled Kamal and Zhang, Xuan and Huang, Qianying and Dubost, Florian and Rubin, Daniel and Lee-Messer, Christopher},
  booktitle={International Conference on Learning Representations},
  year={2021}
}
@article{martini2021deep,
  title={Deep anomaly detection of seizures with paired stereoelectroencephalography and video recordings},
  author={Martini, Michael L and Valliani, Aly A and Sun, Claire and Costa, Anthony B and Zhao, Shan and Panov, Fedor and Ghatan, Saadi and Rajan, Kanaka and Oermann, Eric Karl},
  journal={Scientific Reports},
  volume={11},
  number={1},
  pages={1--11},
  year={2021},
  publisher={Nature Publishing Group}
}
@inproceedings{xu2020anomaly,
  title={Anomaly Detection on Electroencephalography with Self-supervised Learning},
  author={Xu, Junjie and Zheng, Yaojia and Mao, Yifan and Wang, Ruixuan and Zheng, Wei-Shi},
  booktitle={2020 IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
  pages={363--368},
  year={2020},
  organization={IEEE}
}
@article{jing2020self,
  title={Self-supervised visual feature learning with deep neural networks: A survey},
  author={Jing, Longlong and Tian, Yingli},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={43},
  number={11},
  pages={4037--4058},
  year={2020},
  publisher={IEEE}
}
@article{manna,
	title={Neural correlates of focused attention and cognitive monitoring in meditation},
	author={Manna, Antonietta and Raffone, Antonino and Perrucci, Mauro Gianni and Nardo, Davide and Ferretti, Antonio and Tartaro, Armando and Londei, Alessandro and Del Gratta, Cosimo and Belardinelli, Marta Olivetti and Romani, Gian Luca},
	journal={Brain research bulletin},
	volume={82},
	number={1-2},
	pages={46--56},
	year={2010},
	publisher={Elsevier}
}

@misc{WHO2019, 
	title={Epilepsy}, url={https://www.who.int/news-room/fact-sheets/detail/epilepsy}, 
	journal={World Health Organization}, 
	publisher={World Health Organization}
} 
@misc{lecun_2019, title={I'm giving the introductory keynote at the International Solid State Circuit Conference in San Francisco This Morning at 8:45 PST.Slides here: Https://t.co/uqyx4hphyl}, url={https://twitter.com/ylecun/status/1097532314614034433}, journal={Twitter}, publisher={Twitter}, author={LeCun, Yann}, year={2019}, month={Feb}
} 
@article{jing2020self,
	title={Self-supervised visual feature learning with deep neural networks: A survey},
	author={Jing, Longlong and Tian, Yingli},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	volume={43},
	number={11},
	pages={4037--4058},
	year={2020},
	publisher={IEEE}
}
@article{shah2018temple,
	title={The temple university hospital seizure detection corpus},
	author={Shah, Vinit and Von Weltin, Eva and Lopez, Silvia and McHugh, James Riley and Veloso, Lillian and Golmohammadi, Meysam and Obeid, Iyad and Picone, Joseph},
	journal={Frontiers in neuroinformatics},
	volume={12},
	pages={83},
	year={2018},
	publisher={Frontiers}
}
@incollection{asif2020seizurenet,
	title={SeizureNet: Multi-spectral deep feature learning for seizure type classification},
	author={Asif, Umar and Roy, Subhrajit and Tang, Jianbin and Harrer, Stefan},
	booktitle={Machine Learning in Clinical Neuroimaging and Radiogenomics in Neuro-oncology},
	pages={77--87},
	year={2020},
	publisher={Springer}
}
@article{ahmedt2020identification,
	title={Identification of children at risk of schizophrenia via deep learning and EEG responses},
	author={Ahmedt-Aristizabal, David and Fernando, Tharindu and Denman, Simon and Robinson, Jonathan Edward and Sridharan, Sridha and Johnston, Patrick J and Laurens, Kristin R and Fookes, Clinton},
	journal={IEEE journal of biomedical and health informatics},
	volume={25},
	number={1},
	pages={69--76},
	year={2020},
	publisher={IEEE}
}

@article{li2017diffusion,
	title={Diffusion convolutional recurrent neural network: Data-driven traffic forecasting},
	author={Li, Yaguang and Yu, Rose and Shahabi, Cyrus and Liu, Yan},
	journal={arXiv preprint arXiv:1707.01926},
	year={2017}
}
@article{rasheed2020machine,
	title={Machine learning for predicting epileptic seizures using EEG signals: A review},
	author={Rasheed, Khansa and Qayyum, Adnan and Qadir, Junaid and Sivathamboo, Shobi and Kwan, Patrick and Kuhlmann, Levin and O’Brien, Terence and Razi, Adeel},
	journal={IEEE Reviews in Biomedical Engineering},
	volume={14},
	pages={139--155},
	year={2020},
	publisher={IEEE}
}
@article{chami2020machine,
	title={Machine learning on graphs: A model and comprehensive taxonomy},
	author={Chami, Ines and Abu-El-Haija, Sami and Perozzi, Bryan and R{\'e}, Christopher and Murphy, Kevin},
	journal={arXiv preprint arXiv:2005.03675},
	year={2020}
}
@article{bronstein2017geometric,
	title={Geometric deep learning: going beyond euclidean data},
	author={Bronstein, Michael M and Bruna, Joan and LeCun, Yann and Szlam, Arthur and Vandergheynst, Pierre},
	journal={IEEE Signal Processing Magazine},
	volume={34},
	number={4},
	pages={18--42},
	year={2017},
	publisher={IEEE}
}
@article{saab2020weak,
	title={Weak supervision as an efficient approach for automated seizure detection in electroencephalography},
	author={Saab, Khaled and Dunnmon, Jared and R{\'e}, Christopher and Rubin, Daniel and Lee-Messer, Christopher},
	journal={NPJ digital medicine},
	volume={3},
	number={1},
	pages={1--12},
	year={2020},
	publisher={Nature Publishing Group}
}
@inproceedings{ahmedt2020neural,
	title={Neural memory networks for seizure type classification},
	author={Ahmedt-Aristizabal, David and Fernando, Tharindu and Denman, Simon and Petersson, Lars and Aburn, Matthew J and Fookes, Clinton},
	booktitle={2020 42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
	pages={569--575},
	year={2020},
	organization={IEEE}
}
@article{kostas2021bendr,
	title={BENDR: using transformers and a contrastive self-supervised learning task to learn from massive amounts of EEG data},
	author={Kostas, Demetres and Aroca-Ouellette, Stephane and Rudzicz, Frank},
	journal={Frontiers in Human Neuroscience},
	volume={15},
	year={2021},
	publisher={Frontiers Media SA}
}
@article{hopp2016,
	title={Electroencephalography (EEG): An Introductory Text and Atlas of Normal and Abnormal Findings in Adults, Children, and Infants [Internet]},
	journal = {Chicago: American Epilepsy Society},
	year = {2016},
	site= {The Normal EEG. Available from: https://www.ncbi.nlm.nih.gov/books/NBK390343/}
}
@article{hiraoka1980,
	author = {Hiraoka, M},
	year = {1980},
	month = {01},
	pages = {2184-90},
	title = {Physiological study of the Bell's phenomenon in human (Japa)},
	volume = {83},
	journal = {Nippon Ganka Gakkai zasshi}
}
@article{bromfield2006,
	title={An Introduction to Epilepsy},
	journal = {Chicago: American Epilepsy Society},
	key = {National library of medicine},
	year = {2006},
	site= {https://www.ncbi.nlm.nih.gov/books/NBK2508/}
}
@inproceedings{doersch2015unsupervised,
  title={Unsupervised visual representation learning by context prediction},
  author={Doersch, Carl and Gupta, Abhinav and Efros, Alexei A},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1422--1430},
  year={2015}
}
@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}
@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}
@article{grill2020bootstrap,
  title={Bootstrap your own latent-a new approach to self-supervised learning},
  author={Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre and Buchatskaya, Elena and Doersch, Carl and Avila Pires, Bernardo and Guo, Zhaohan and Gheshlaghi Azar, Mohammad and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={21271--21284},
  year={2020}
}
@article{lan2019albert,
  title={Albert: A lite bert for self-supervised learning of language representations},
  author={Lan, Zhenzhong and Chen, Mingda and Goodman, Sebastian and Gimpel, Kevin and Sharma, Piyush and Soricut, Radu},
  journal={arXiv preprint arXiv:1909.11942},
  year={2019}
}
@article{bai2020representation,
  title={Representation learning for sequence data with deep autoencoding predictive components},
  author={Bai, Junwen and Wang, Weiran and Zhou, Yingbo and Xiong, Caiming},
  journal={arXiv preprint arXiv:2010.03135},
  year={2020}
}

@article{arora2019theoretical,
  title={A theoretical analysis of contrastive unsupervised representation learning},
  author={Arora, Sanjeev and Khandeparkar, Hrishikesh and Khodak, Mikhail and Plevrakis, Orestis and Saunshi, Nikunj},
  journal={arXiv preprint arXiv:1902.09229},
  year={2019}
}
@article{lee2021predicting,
  title={Predicting what you already know helps: Provable self-supervised learning},
  author={Lee, Jason D and Lei, Qi and Saunshi, Nikunj and Zhuo, Jiacheng},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}
@article{wei2020theoretical,
  title={Theoretical analysis of self-training with deep networks on unlabeled data},
  author={Wei, Colin and Shen, Kendrick and Chen, Yining and Ma, Tengyu},
  journal={arXiv preprint arXiv:2010.03622},
  year={2020}
}
@article{saunshi2020mathematical,
  title={A mathematical exploration of why language models help solve downstream tasks},
  author={Saunshi, Nikunj and Malladi, Sadhika and Arora, Sanjeev},
  journal={arXiv preprint arXiv:2010.03648},
  year={2020}
}
@article{smith2005eeg,
  title={EEG in the diagnosis, classification, and management of patients with epilepsy},
  author={Smith, Shelagh JM},
  journal={Journal of Neurology, Neurosurgery \& Psychiatry},
  volume={76},
  number={suppl 2},
  pages={ii2--ii7},
  year={2005},
  publisher={BMJ Publishing Group Ltd}
}
@article{ebersole1983evaluation,
  title={Evaluation of ambulatory cassette EEG monitoring: III. Diagnostic accuracy compared to intensive inpatient EEG monitoring},
  author={Ebersole, John S and Leroy, Robert F},
  journal={Neurology},
  volume={33},
  number={7},
  pages={853--853},
  year={1983},
  publisher={AAN Enterprises}
}
@inproceedings{varatharajah2020electrophysiological,
  title={Electrophysiological correlates of brain health help diagnose epilepsy and lateralize seizure focus},
  author={Varatharajah, Yogatheesan and Berry, Brent and Joseph, Boney and Balzekas, Irena and Kremen, Vaclav and Brinkmann, Benjamin and Worrell, Gregory and Iyer, Ravishankar},
  booktitle={2020 42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  pages={3460--3464},
  year={2020},
  organization={IEEE}
}
@article{obeid2016temple,
  title={The temple university hospital EEG data corpus},
  author={Obeid, Iyad and Picone, Joseph},
  journal={Frontiers in neuroscience},
  volume={10},
  pages={196},
  year={2016},
  publisher={Frontiers}
}
@article{gramfort2013meg,
  title={MEG and EEG data analysis with MNE-Python},
  author={Gramfort, Alexandre and Luessi, Martin and Larson, Eric and Engemann, Denis A and Strohmeier, Daniel and Brodbeck, Christian and Goj, Roman and Jas, Mainak and Brooks, Teon and Parkkonen, Lauri and others},
  journal={Frontiers in neuroscience},
  pages={267},
  year={2013},
  publisher={Frontiers}
}
@article{hughes2008gamma,
  title={Gamma, fast, and ultrafast waves of the brain: their relationships with epilepsy and behavior},
  author={Hughes, John R},
  journal={Epilepsy \& Behavior},
  volume={13},
  number={1},
  pages={25--31},
  year={2008},
  publisher={Elsevier}
}
@article{parra2003gamma,
  title={Gamma-band phase clustering and photosensitivity: is there an underlying mechanism common to photosensitive epilepsy and visual perception?},
  author={Parra, J and Kalitzin, SN and Iriarte, J and Blanes, W and Velis, DN and Lopes da Silva, FH},
  journal={Brain},
  volume={126},
  number={5},
  pages={1164--1172},
  year={2003},
  publisher={Oxford University Press}
}
@article{medvedev2011abnormal,
  title={Abnormal interictal gamma activity may manifest a seizure onset zone in temporal lobe epilepsy},
  author={Medvedev, Andrei V and Murro, Anthony M and Meador, Kimford J},
  journal={International journal of neural systems},
  volume={21},
  number={02},
  pages={103--114},
  year={2011},
  publisher={World Scientific}
}
@article{ullah2018automated,
  title={An automated system for epilepsy detection using EEG brain signals based on deep learning approach},
  author={Ullah, Ihsan and Hussain, Muhammad and Aboalsamh, Hatim and others},
  journal={Expert Systems with Applications},
  volume={107},
  pages={61--71},
  year={2018},
  publisher={Elsevier}
}
@article{abdelhameed2021deep,
  title={A deep learning approach for automatic seizure detection in children with epilepsy},
  author={Abdelhameed, Ahmed and Bayoumi, Magdy},
  journal={Frontiers in Computational Neuroscience},
  volume={15},
  pages={29},
  year={2021},
  publisher={Frontiers}
}
@article{gleichgerrcht2018deep,
  title={Deep learning applied to whole-brain connectome to determine seizure control after epilepsy surgery},
  author={Gleichgerrcht, Ezequiel and Munsell, Brent and Bhatia, Sonal and Vandergrift III, William A and Rorden, Chris and McDonald, Carrie and Edwards, Jonathan and Kuzniecky, Ruben and Bonilha, Leonardo},
  journal={Epilepsia},
  volume={59},
  number={9},
  pages={1643--1654},
  year={2018},
  publisher={Wiley Online Library}
}
@inproceedings{inproceedings,
author = {Wang, Jialin and Liang, Shen and He, Dake and Wang, Ye and Wu, Yingpei and Zhang, Yanchun},
year = {2020},
month = {12},
pages = {785-792},
title = {A Sequential Graph Convolutional Network with Frequency-domain Complex Network of EEG Signals for Epilepsy Detection},
doi = {10.1109/BIBM49941.2020.9313232}

}@article{varatharajah2017eeg,
  title={EEG-GRAPH: a factor-graph-based model for capturing spatial, temporal, and observational relationships in electroencephalograms},
  author={Varatharajah, Yogatheesan and Chong, Min Jin and Saboo, Krishnakant and Berry, Brent and Brinkmann, Benjamin and Worrell, Gregory and Iyer, Ravishankar},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}
@article{song2018eeg,
  title={EEG emotion recognition using dynamical graph convolutional neural networks},
  author={Song, Tengfei and Zheng, Wenming and Song, Peng and Cui, Zhen},
  journal={IEEE Transactions on Affective Computing},
  volume={11},
  number={3},
  pages={532--541},
  year={2018},
  publisher={IEEE}
}
@inproceedings{wang2018eeg,
  title={EEG emotion recognition using dynamical graph convolutional neural networks and broad learning system},
  author={Wang, Xue-han and Zhang, Tong and Xu, Xiang-min and Chen, Long and Xing, Xiao-fen and Chen, CL Philip},
  booktitle={2018 IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
  pages={1240--1244},
  year={2018},
  organization={IEEE}
}
@inproceedings{aliyu2019epilepsy,
  title={Epilepsy detection in EEG signal using recurrent neural network},
  author={Aliyu, Ibrahim and Lim, Yong Beom and Lim, Chang Gyoon},
  booktitle={Proceedings of the 2019 3rd International Conference on Intelligent Systems, Metaheuristics \& Swarm Intelligence},
  pages={50--53},
  year={2019}
}
@inproceedings{niederhofer2003pattern,
  title={Pattern detection by CNN in epilepsy: recent results},
  author={Niederhofer, Christian and Fischer, Philipp and Tetzlaff, Ronald},
  booktitle={Bioengineered and Bioinspired Systems},
  volume={5119},
  pages={265--272},
  year={2003},
  organization={SPIE}
}
@inproceedings{cho-etal-2014-properties,
    title = "On the Properties of Neural Machine Translation: Encoder{--}Decoder Approaches",
    author = {Cho, Kyunghyun  and
      van Merri{\"e}nboer, Bart  and
      Bahdanau, Dzmitry  and
      Bengio, Yoshua},
    booktitle = "Proceedings of {SSST}-8, Eighth Workshop on Syntax, Semantics and Structure in Statistical Translation",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W14-4012",
    doi = "10.3115/v1/W14-4012",
    pages = "103--111",
}
